Coalition Formation in Constant Sum Queueing Games

We analyse a coalition formation game between strategic service providers of a congestible service. The key novelty of our formulation is that it is a constant sum game, i.e., the total payoff across all service providers (or coalitions of providers) is fixed, and dictated by the total size of the market. The game thus captures the tension between resource pooling (to benefit from the resulting statistical economies of scale) and competition between coalitions over market share. In a departure from the prior literature on resource pooling for congestible services, we show that the grand coalition is in general not stable, once we allow for competition over market share. Instead, the stable configurations are duopolies, where the dominant coalition exploits its economies of scale to corner a disproportionate market share. We analyse the stable duopolies that emerge from this interaction, and also study a dynamic variant of this game.

==> Shiksha.tex <==

\subsection{Two partitions}  We are now left with 2-partitions.  
In this section we derive the configurations  using    2-partitions  that are  possibly stable. We also discuss the payoff vectors that render them stable.  

%{\color{red}Let $N := \sum_i N_i$ be the total number of servers of all the  players and} assume  $N_1 \ge N_2 \ge \cdots N_n$, without loss of generality.
 Any 2-partition $\P = \{C_1, C_2\}$ can be  identified uniquely by $k := N_{C_1} $ the number of servers  of its  first coalition.   For simpler notations,  we  let $\lambda_k := \lambda_{C}^\P$, when $N_C = k$,  and this definition is possible because all the servers are identical. 
Our aim now  is to find  the values of  $k$ that renders the 2-partition stable. 

Let $\Psi(k ; \Lambda)$ represent $\lambda_k / k$ for any given $\Lambda$. By Theorem \ref{Thm_WE},   the function $\Psi(k ; \Lambda)$  equals $1/k$ times the unique  zero  of the following function  of $\lambda$ (see \eqref{Eqn_WE_properties}):
$$
h(\lambda) :=   \frac { \lambda^k } { k! }   \sum_{j=0}^{N-k} \frac{ (\Lambda-\lambda)^j }{j!}   -  \frac{{(\Lambda-\lambda)}^{N-k}}{(N-k)!}     \sum_{j=0}^{k} \frac{\lambda^j} {j!}.
 $$
 Observe here that $\lambda_{N-k} = \Lambda - \lambda_k$. 

 We immediately have the following:
 \begin{theorem}
{\bf [Stable configuration under rule-A]} 
\label{Thm_two_partition}
i) The value of $k$  that renders the  partition $\P = \{S,  {\cal N}\backslash S\}$ (with $|S| = k$)   stable  is given  by:
\begin{eqnarray}
 k^* (\Lambda) := \arg \max_{k: k = N_C, C \subset {\cal N} }   \Psi(k ; \Lambda). \label{Eqn_kstar}
\end{eqnarray}


ii) If in any 2-partition $\P = \{C_1,C_2\}$, there exists no coalition $S \subset C_i \text{ for } i=\{1,2\}$ such that equation \eqref{Eqn_condition_S} is satisfied, then such a 2-partition is also stable.
\\
Both the results are true irrespective of the   payoff vector $\Phi^\P.$
\label{Thm_Prule_stability}
\end{theorem}
{\bf Proof:} See Appendix B. \eop




\subsection{Anticipation  rule-B}  The equations \eqref{Eqn_condition_M}-\eqref{Eqn_condition_S} can be seen as the  initial anticipation/assessment  by the new coalition before plunging into the action.  They consider pessimal rule for anticipation to safeguard themselves from future mergers/coalitions.  The merger/split will really  be through if further equation \eqref{Eqn_Example_fair_rule_M} and \eqref{Eqn_Example_fair_rule_S} is satisfied, and one can view this as final assessment after further fact-checking.  

Alternatively one can consider one step anticipation rule, in which a new  coalition $Q$ (merger/split) is formed if the following is satisfied:
\begin{eqnarray}
\label{Eqn_alternate_rule}
\ulam_Q  >  \sum_{i \in Q}  \phi_i^\P  .
\end{eqnarray}
Note by definition of $\ulam_Q$, under this anticipation rule, the new coalition always perform superior (as $\ulam_Q \le \lambda_Q^{\P'} $ for all $\P'$) and hence can be seen as one step assessment.  

Interestingly under this condition, there exists stable coalitions that are dependent on the payoff vector $\Phi^{\P}$. We say the payoff vector $\Phi^{\P}_p$ to be \textit{proportional} if  the share of  value of any coalition (in any partition)  to any of its members is   proportional to value of its resources divided by the total value of the resources of all the members of the coalition. For example, in our queueing model:
\begin{eqnarray}
\label{Eqn_PSA}
\phi^{\P}_{p, i}  =  \frac{N_i}{ \sum_{j \in C} N_j }   \lambda_C^\P \mbox{ for any } i  \in C \in \P.
\end{eqnarray}:
\begin{theorem}{\bf [(Un)Stable configurations under rule-B]}
\label{Thm_stable_config_ruleB}
i)  There exist no  payoff vector under anticipation rule-B \eqref{Eqn_alternate_rule} that  renders GC stable.

ii) Partitions of size more than two are never a part of the stable configuration. 

ii) The configuration $(\P, \Phi_p^\P)$ is stable under rule-B, where  $\P = \{S, \mathcal{N}\backslash S\}$  is any stable    2-partition of   Theorem \ref{Thm_two_partition}  and $\Phi_p^\P$  is the  PF  payoff vector corresponding to $\P$  defined by \eqref{Eqn_PSA}. 
 
%All the partitions are unstable irrespective of the allocation vectors under the anticipation rule \eqref{Eqn_alternate_rule}.
\label{Thm_R_rule_stability}
\end{theorem}
\textbf{Proof:} See Appendix B. \eop


